Zero-shot Generalizable Incremental Learning for Vision-Language Object Detection

This paper presents Incremental Vision-Language Object Detection (IVLOD), a novel learning task designed to incrementally adapt pre-trained Vision-Language Object Detection Models (VLODMs) to various specialized domains, while simultaneously preserving their zero-shot generalization capabilities for the generalized domain. To address this new challenge, we present the Zero-interference Reparameterizable Adaptation (ZiRa), a novel method that introduces Zero-interference Loss and reparameterization techniques to tackle IVLOD without incurring additional inference costs or a significant increase in memory usage. Comprehensive experiments on COCO and ODinW-13 datasets demonstrate that ZiRa effectively safeguards the zero-shot generalization ability of VLODMs while continuously adapting to new tasks. Specifically, after training on ODinW-13 datasets, ZiRa exhibits superior performance compared to CL-DETR and iDETR, boosting zero-shot generalizability by substantial 13.91 and 8.74 AP, respectively.Our code is available at https://github.com/JarintotionDin/ZiRaGroundingDINO.

==> sec/2_relat_back.tex <==
\section{Related Work}
\label{sec:relat}
\textbf{Vision-Language Object Detection.}
Vision-Language Object Detection Models (VLODMs) combine natural language descriptions with object detection in images. Early research in this area primarily focused on grounding textual phrases to image regions, such as grounding referring expressions \cite{DBLP:conf/cvpr/MaoHTCY016, DBLP:journals/pami/YangLY21, DBLP:journals/pami/DengWWHLT22} and visual question answering \cite{DBLP:conf/cvpr/00010BT0GZ18, DBLP:conf/nips/LuBPL19, DBLP:conf/cvpr/Yu0CT019}. More recent studies have developed unified and scalable approaches for simultaneous object detection and grounding tasks. For instance, GLIP \cite{DBLP:conf/cvpr/LiZZYLZWYZHCG22} unifies phrase grounding and object detection tasks by treating object detection as context-free phrase grounding and treating phrase grounding as a contextualized object detection task. This approach enables the integration of multi-layered textual information into the detection model. Grounding DINO \cite{DBLP:journals/corr/abs-2303-05499}, based on the DINO \cite{DBLP:conf/iclr/0097LL000NS23}, employs a DETR-like \cite{DBLP:conf/eccv/CarionMSUKZ20} architecture that uses a Transformer as the detector, which allows for unified processing of image and language data and offers the outstanding capacity to utilize large-scale datasets. Based on Grounding DINO, our work further addresses the newly introduced IVLOD tasks.

\textbf{Incremental Learning.}
Incremental learning, also known as continual learning or lifelong learning, tackles the challenge of learning new tasks without forgetting previous ones. Incremental learning has given rise to two primary strategies, memory replay, and knowledge distillation, to tackle its inherent challenges \cite{DBLP:conf/eccv/LiH16, DBLP:conf/cvpr/RebuffiKSL17, DBLP:conf/cvpr/CermelliMB0C20, DBLP:journals/corr/abs-2204-03410, DBLP:conf/cvpr/0002ZL0SRSPDP22, DBLP:journals/corr/abs-2207-12819, DBLP:conf/iccv/0002LLZWHMHL23}. For example, Learning without Forgetting (LwF) \cite{DBLP:conf/eccv/LiH16} employs knowledge distillation to maintain performance on old tasks while learning new ones. Another notable approach, iCaRL \cite{DBLP:conf/cvpr/RebuffiKSL17}, combines exemplar memory and a nearest-mean-of-exemplars classification method for incremental learning.

\textbf{Incremental Object Detection.}
Incremental object detection, a specialized subfield within incremental learning, focuses on improving the adaptability of object detection models to new object categories while maintaining performance on previously learned categories \cite{DBLP:conf/iccv/ShmelkovSA17, DBLP:journals/pami/JosephRKKB22, DBLP:conf/cvpr/Perez-RuaZHX20, DBLP:conf/cvpr/YinPL22, DBLP:conf/cvpr/GaneaBP21, DBLP:conf/aaai/Dong0DL23, DBLP:conf/cvpr/0001SV023}. ILOD \cite{DBLP:conf/iccv/ShmelkovSA17} was the first to introduce incremental object detection. More recently, CL-DETR \cite{DBLP:conf/cvpr/0001SV023} effectively combined knowledge distillation and exemplar memory techniques to enhance incremental object detection using Transformer-based models. Our work distinguishes itself by performing incremental learning on VLODMs, which are more favorable for open-world problems. Besides the need to continually adapt across multiple specialized tasks, it is also important to preserve their zero-shot generalization ability. To the best of our knowledge, our work is the first to pose and tackle IVLOD tasks. 

\textbf{Reparameterization.}
Reparameterization techniques optimize model inference speed by transforming the training-time architecture into an equivalent, simplified form for inference \cite{DBLP:conf/iccv/DingGDH19, DBLP:conf/cvpr/Ding0MHD021, DBLP:conf/cvpr/DingC0HD22}. RepVGG \cite{DBLP:conf/cvpr/Ding0MHD021} exemplified this approach by employing $3\times3$ and $1\times1$ convolutional branches for training, which are streamlined to $3\times3$ convolutional branches and ReLU activations during inference. RepMLPNet \cite{DBLP:conf/cvpr/DingC0HD22} introduced ``Locality Injection" to merge trained parameters of parallel convolutional kernels into fully connected layers, enhancing MLP-based model performance. Our work builds upon the Reparameterizable Dual Branch (RDB) concept initially proposed by \cite{DBLP:conf/cvpr/ZhangXLCC22}. The key innovations introduced in our approach include the use of differentiated learning rates for the High Learning Rate Branch and Low Learning Rate Branch, and the implementation of Zero-interference Loss (ZiL). These enhancements allow for a more effective balance between learning new tasks and preserving previously acquired knowledge, distinguishing our method from prior work.

